Leveraging Affective Bidirectional Transformers for Offensive Language Detection

Social media are pervasive in our life, making it necessary to ensure safe online experiences by detecting and removing offensive and hate speech. In this work, we report our submission to the Offensive Language and hate-speech Detection shared task organized with the 4th Workshop on Open-Source Arabic Corpora and Processing Tools Arabic (OSACT4). We focus on developing purely deep learning systems, without a need for feature engineering. For that purpose, we develop an effective method for automatic data augmentation and show the utility of training both offensive and hate speech models off (i.e., by fine-tuning) previously trained affective models (i.e., sentiment and emotion). Our best models are significantly better than a vanilla BERT model, with 89.60% acc (82.31% macro F1) for hate speech and 95.20% acc (70.51% macro F1) on official TEST data.

==> to_do.tex <==
Ask Moatez: 

1. To get some stats as to how many tweets have we acquired per query word.

2. To get a TSV file with each query word and its tweet ids (two columns, with second column for all tweet ids, comma separated), while the two main columns are separated by a tab.

3. Train a word2vec model.


